CIZSL++: Creativity Inspired Generative Zero-Shot Learning

Zero-shot learning (ZSL) aims at understanding unseen categories with no training examples from class-level descriptions. To improve the discriminative power of ZSL, we model the visual learning process of unseen categories with inspiration from the psychology of human creativity for producing novel art. First, we propose CIZSL-v1 as a creativity inspired model for generative ZSL. We relate ZSL to human creativity by observing that ZSL is about recognizing the unseen, and creativity is about creating a likable unseen. We introduce a learning signal inspired by creativity literature that explores the unseen space with hallucinated class-descriptions and encourages careful deviation of their visual feature generations from seen classes while allowing knowledge transfer from seen to unseen classes. Second, CIZSL-v2 is proposed as an improved version of CIZSL-v1 for generative zero-shot learning. CIZSL-v2 consists of an investigation of additional inductive losses for unseen classes along with a semantic guided discriminator. Empirically, we show consistently that CIZSL losses can improve generative ZSL models on the challenging task of generalized ZSL from a noisy text on CUB and NABirds datasets. We also show the advantage of our approach to Attribute-based ZSL on AwA2, aPY, and SUN datasets. We also show that CIZSL-v2 has improved performance compared to CIZSL-v1.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TODO-Kai.tex <==
% \section{TODO Next}
% \begin{itemize}
%     \item Finish a cover letter to show the difference between the conference submission and the journal submission.
%     \item Try to have some similar figures like Fig 7, maybe also Fig 6 in the Link the head paper.
%     \item Read the paper \textit{Class Normalization for Zero-Shot Learning} to see what I can do later.
% \end{itemize}

\section*{Cover Letter}
% TODO: talk about the conference submission details.

\begin{enumerate}
    % \item This is to show the difference between the conference submission and the journal submission.
    \item \textbf{Hyperparameters selection} In our journal submission, we made extensive hyperparameters selection based on the optimal conference paper. We found the best hyperparameters selection is consistent.
    \item \textbf{Network architectures} In our journal submission, we extend the simple and basic MLP generator/discriminator to more complex DoubleNet and reduced dimensional DoubleNet. Experimental results show the simple (original) design works best.
    \item \textbf{Hallucinated text generation strategy} In our previous conference submission, $t^h$ is generated by $\alphat^s_a + (  -\alpha)t^s_b, \alpha \in \mathcal{U}(0.2, 0.8)$. While in our journal version, we did extensive interpolations and extrapolations with $\alpha$ uniformly sampled from $(-0.5, -0.2)$, $(0.2, 0.8)$, $(1.2, 1.5)$ and their different combinations. Experimental results shows there is no huge different with different hallucinated text generation strategies.
    \item \textbf{Generation loss for the hallucinated text to the discriminator} In our conference version, we only considered the discriminative ability with real image $x$ and generated features given text features of seen classes. In this case, there is no motivation for the discriminator to learn from hallucinated text. Therefore, in our journal version, we apply the creativity loss $L_{G}^{C}=-E_{z \sim p_{x}, t^{h} \sim p_{t e x t}^{x}}\left[D^{r}\left(G\left(t^{h}, z\right)\right)\right]$ $+\lambda E_{z \sim p_{z}, t^{h} \sim p_{t e x t}^{h}}\left[L_{e}\left(\left\{D^{s, k}\left(G\left(t^{h}, z\right)\right)\right\}_{k=1 \rightarrow K^{\alpha}}\right)\right]$ to make the discriminator to discriminate the hallucinated text. Experimental results show the proposed loss does not help.
    \item \textbf{Semantically Guided Categorizer (SeGC)} In our conference submission, we use the classification head modeled by the cross-entropy loss to guide the generator to generate more realistic images but not pushing so far. In our journal extension, we replace the classification head at the discriminator with a novel semantically guided discriminator, which leverage the generated image features and their corresponding semantic features from different types (i.e., hallucinated text, seen text). Extensive experiments show our proposed SeGC can significantly improve the performance.
    \item \textbf{Scaled normalization of SeGC} In our journal extension, we normalize the inputs of SeGC with different scaling factors. Experimental results show the scaled normalization strategy is not helpful for SeGC.
    \item \textbf{Adding hallucinated real-fake loss for the discriminator}  In our journal version, we add the hallucinated real-fake loss for the discriminator. Experimental results show the added loss can improve the performance.
    \item \textbf{Categorization on hallucinated visual features of hallucinated text} In our journal extension, we explicitly constrain the class number for hallucinated text (i.e., 10, 20, 50, 100, the original number is 1000); we found the class number equals 100 works better. However, adding the categorization loss of hallucinated text do not improve the performance.
    % \item \textbf{Part-to-Term connectivity} Based on the link-to-head Fig. 7 and Fig. 6. TODO Next.
\end{enumerate}  
  
\begin{table}[!htbp]
    \centering
    \begin{tabular}{p{0.2\columnwidth}|p{0.35\columnwidth}|p{0.35\columnwidth}}
        \toprule
        Item & Conference Submission & Journal Submission \\ \midrule
        Hyperparameters selection & Limited testing on the creativity weight & Extensive experiments on hyperparameters (creativity weight, learning rate, training epochs)\\ \midrule
        Network architectures & Simple and basic MLP implementations & More evaluations on DoubleNet and reduced dim DoubleNet\\ \midrule
        Hallucinated text generation strategy & Interpolation from two seen text description with an interpolation factor sampled from $\mathcal{U}(0.2, 0.8)$ & Try interpolation/extrapolation factors sampled from different distributions\\ \midrule
        Generation loss for the hallucinated text to the discriminator & Not applied & Applied and did extensive experiments on this loss\\ \midrule
        Semantically Guided Discriminator (SeGC) & Not applied & Did extensive experiments on this loss for text-based dataset and show SeGC cam improve the performance\\ \midrule
        Scaled normalization of SeGC & Not applied & Did normalization of SeGC with different scale factors\\ \midrule
        Adding hallucinated real-fake loss for the discriminator & Not applied & Add this loss and did extensive studies\\ \midrule
        Categorization on hallucinated visual features of hallucinated text & Not applied & Add the categorization on hallucinated visual features\\
        % Part-to-Term connectivity (\textbf{TODO}) & Not applied & TODO\\
        \bottomrule
    \end{tabular}
    \caption*{Cover Letter to show the difference between the conference submission and the journal submission.}
    \label{tab:cover-letter}
\end{table}

% Update: Dec. 26th, 2020, 11am Beijing Time.  

==> exp-old.tex <==




%\mohamed{Rememeber to add Generator and Discriminator architecture details in Supplementary}



We investigate the performance of our approach on two class-level semantic settings: textual  and attribute descriptions. Since the textual based ZSL is a harder problem, we used it to run an ablation study for  zero-shot retrieval and generalized ZSL. Then, we conducted  experiments for both settings to validate the generality of our work.

\noindent \textbf{Cross-Validation} 
The weight $\lambda$ of our loss in Eq~\ref{eq_lgc} is a hyperparameter  that we found easy to tune on all of our experiments. %For our experiments, we perform cross-validation to obtain the value of $\lambda$ that varies by setting.
We start by splitting the data into training and validation split with nearly 80-20\% ratio for all settings. Training and validation classes are selected randomly prior to the training. Then, we compute validation performance when training the model on the 80\% split every 100 iterations out of 3000 iterations. We investigate a wide range of values for $\lambda$, and the value that scores highest validation performance is selected to be used at the inference time. Finally, we combine training and validation data and evaluate the performance on testing data.


\noindent \textbf{Zer-Shot Performance Metrics.} We use two metrics widely used in in evaluating ZSL recognition performance: Standard Zero-shot recognition with the Top-1 unseen class accuracy and Seen-Unseen Generalized Zero-shot performance with Area under Seen-Unseen curve~\cite{chao2016empirical}. The Top-1 accuracy is the average percentage   of  images from unseen classes classifying correctly to one of unseen class labels. However, this might be  incomplete measure since it is more realistic at inference time to encounter also seen classes. Therefore, We also report a generalized zero-shot recognition metric with respect to the seen-unseen  curve, proposed by Chao~\emph{et al.}~\cite{chao2016empirical}. This metric classifies images of both seen $\mathcal{S}$ and unseen classes $\mathcal{U}$ at test time. Then, the performance of a ZSL model is assessed by classifying these images to the label space that covers both seen classes and unseen labels $\mathcal{T} = \mathcal{S}\cup\mathcal{U}$. A balancing parameter is used sample seen and unseen class test accuracy-pair. This pair is plotted as the $(x,y)$ co-ordinate to form the Seen-Unseen Curve(SUC). We follow ~\cite{Elhoseiny_2018_CVPR} in using the Area Under SUC to evaluate the generalization capability of class-level text zero-shot recognition, and the haromnic mean of SUC for attribute-based zero-shot recognition. In our model, we use the trained GAN to synthesize the visual features for both training and testing classes.

\begin{table*}[!htbp]
% \vspace{-4mm}
\parbox{.60\linewidth}{
\centering
\resizebox{.60\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
\textbf{CIZSL SM-Entropy (ours final)} & \textbf{44.6} & \textbf{14.4} & 36.5 & \textbf{9.3} &  & \textbf{39.2} & \textbf{11.9} & \textbf{24.5} & \textbf{6.4} \\ \hline 
CIZSL SM-Entropy (replace $2^{nd}$ term in Eq~\ref{eq_lgc} by Classifying $t^h$ as new class) & 43.2 & 11.31 & 35.6 & 8.5 &  &38.3 & 9.5 & 21.6 & 5.6\\ 
CIZSL SM-Entropy (minus  $1^{st}$ term in Eq~\ref{eq_lgc}) & 43.4 & 10.1 & 35.2 & 8.3 &  & 35.0 & 8.2 & 20.1  & 5.4\\  
CIZSL SM-Entropy: (minus  $2^{nd}$ term in Eq~\ref{eq_lgc}) & 41.7 & 11.2 & 33.4 & 8.1 &  & 33.3 & 10.1 & 21.3 & 5.1\\
\hline 
CIZSL Bachatera-Entropy ($\gamma=0.5,\beta =0.5$) & 44.1 & 13.7 & 35.9 & 8.9 &  & 38.9 & 10.3 & 24.3 & 6.2\\
CIZSL Renyi-Entropy ($\beta \to 1$) &  44.1 & 13.3 & 35.8 & 8.8 &  & 38.6 & 10.3 & 23.7 & 6.3\\	
CIZSL KL-Entropy ($\gamma \to 1,\beta \to 1$)	&  44.5 & 14.2 & 36.3 & 8.9 &  & 38.9 & 11.6 & 24.3 & 6.2\\
CIZSL Tsallis-Entropy ($\beta = \gamma$) & 44.1 & 13.8 & \textbf{36.7} & 8.9 &  & 38.9 & 11.3 & 24.5 & 6.3  \\	  \hline
CIZSL SM-Entropy: (minus  $1^{st}$ and $2^{nd}$ terms in Eq~\ref{eq_lgc})= GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\ 
\bottomrule
\end{tabular}%
}
\caption{Ablation Study using Zero-Shot recognition on \textbf{CUB} \& \textbf{NAB} datasets with two split settings each. CIZSL is GAZSL~\cite{Elhoseiny_2018_CVPR}+ our loss}
\label{tb:nab_cub_ablation}
}
\hfill
\parbox{.38\linewidth}{
\centering
\includegraphics[width=0.30\textwidth, height=3.62cm]{img/ParakeetAuklet_vs_CrestedAukletAUC_final.png}
		\vspace{-3mm}
\captionof{figure}{Seen Unseen Curve for Parakeet Auklet (Seen,  y-axis) vs Crested Auklet (Unseen, x-axis) for GAZSL[57] and     GAZSL[57]+ CIZSL.}
\label{fig_auklet}
}
% \vspace{-3.67ex}
\end{table*}


\subsection{Wikipedia based ZSL  Results (4 benchmarks)}
\noindent \textbf{Text Representation.} Textual features for each class are extracted from corresponding raw Wikipedia articles collected by~\cite{elhoseiny2013write,Elhoseiny_2017_CVPR}. %Text articles are first tokenized into words where the stop words are removed. Porter stemmor~\cite{Porter} is applied to reduce inflected words to their word stem.
We used Term Frequency-Inverse Document Frequency (TF-IDF)~\cite{salton1988term} feature vector of dimensionality 7551 for CUB and 13217 for NAB.  %Despite TF-IDF's simplicity, it has been adopted in  the state-of-the-art approaches for this task due to its superiority~\cite{elhoseiny2013write, Qiao2016, Elhoseiny_2017_CVPR}. 

\noindent \textbf{Visual Representation.} We use features of the part-based FC layer in VPDE-net~\cite{zhang2016learning}. The image are fed forward to the VPDE-net after resizing to $224\times 224$, and the feature activation for each detected part is extracted which is of 512 dimensionality. The dimensionalities of visual features for CUB and NAB are 3583 and 3072 respectively. There are six semantic parts shared in CUB and NAB:``head", ``back", ``belly", ``breast", ``leg", ``wing", ``tail". Additionally, CUB has an extra part which is ``leg" which makes its feature representation 512D longer compared to NAB (3583 vs 3072). More details in the Appendix F.
% ; we add more details about the feature extraction in the supplementary. 

\noindent \textbf{Datasets.} We use two common fine-grained recognition datasets for textual descriptions: \emph{Caltech UCSD Birds-2011} (CUB)~\cite{wah2011caltech} and \emph{North America Birds} (NAB)~\cite{Horn2015}. CUB dataset contains 200 classes of bird species and their Wikipedia textual description constituting a total of 11,788 images. Compared to CUB, NAB is a larger dataset of birds, containing a 1011 classes and 48,562 images.

\noindent \textbf{Splits.} For both datasets, there are two schemes to split the classes into training/testing (in total four benchmarks): Super-Category-Shared (SCS) or \textit{easy} split and Super-Category-Exclusive Splitting (SCE) or \textit{hard} split, proposed in~\cite{Elhoseiny_2017_CVPR}. Those splits represents the similarity of the seen to unseen classes, such that the former represents a higher similarity than the latter. For SCS (easy), unseen classes are deliberately picked such that for every unseen class, there is at least one seen class with the same super-category. Hence, the relevance between seen and unseen classes is very high, deeming the zero-shot recognition and retrieval problems relatively easier. On the other end of the spectrum,  SCE (hard) scheme, the unseen classes do not share the super-categories with the seen classes. Hence, there is lower similarity between the seen and unseen classes making the problem harder to solve. Note that the easy split is more common in literature since it is more Natural yet the deliberately designed hard-split shows the progress when the super category is not seen that we also may expect. 

\begin{table*}
\parbox{.57\linewidth}{
\centering
\resizebox{.56\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 & -- & -- &  & 23.9 & 4.9 & 23.5 & -- \\
WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 & 11.4 & 6.0 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 & 24.3 & 6.3 &  & 18.5 & 4.5 & 9.2 & 2.9 \\
ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & 24.5 & 6.8 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & 18.4 & 3.8 &  & 13.1 & 4.0 & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 & -- & -- &  & 1.7 & 1.0 & 0.1 & --\\
ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2 & 9.7 &30.3 & 8.1 &  & 30.4 & 6.1 & 12.6 & 3.5 \\ \hline
FeatGen~\cite{xian2018feature} &  43.9 & 9.8 &36.2 & 8.7 &  & 34.1 & 7.4 & 21.3 & 5.6 \\
FeatGen\cite{xian2018feature}+ \textbf{CIZSL} &  44.2$\mathcolor{blue}{\mathbf{ ^{+0.3}}}$  & 12.1 $\mathcolor{blue}{\mathbf{ ^{+2.3}}}$  & 36.3 $ \mathcolor{blue}{\mathbf{ ^{+0.1}}}$ & \textbf{9.8} $\mathcolor{blue}{\mathbf{ ^{+1.1}}}$ &  & 37.4 $\mathcolor{blue}{\mathbf{ ^{+2.7}}}$ & 9.8$\mathcolor{blue}{\mathbf{ ^{+2.4}}}$ & 24.7$\mathcolor{blue}{\mathbf{ ^{+3.4}}}$ & 6.2 $\mathcolor{blue}{\mathbf{ ^{+0.6}}}$ \\  \hline
GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\    \midrule
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL} &  \textbf{44.6} $\mathcolor{blue}{\mathbf{ ^{+0.9}}}$ & \textbf{14.4} $\mathcolor{blue}{\mathbf{ ^{+4.1}}}$ & \textbf{36.6} $\mathcolor{blue}{\mathbf{ ^{+1.0}}}$ & 9.3 $\mathcolor{blue}{\mathbf{ ^{+0.7}}}$ &  & \textbf{39.2}$\mathcolor{blue}{\mathbf{ ^{+3.8}}}$ & \textbf{11.9}$\mathcolor{blue}{\mathbf{ ^{+3.2}}}$ & \textbf{24.5}$\mathcolor{blue}{\mathbf{ ^{+4.1}}}$ & \textbf{6.4}$\mathcolor{blue}{\mathbf{ ^{+0.6}}}$\\ \bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level textual description from \textbf{CUB} and \textbf{NAB} datasets with two-split setting.}
\label{tb:nab_cub}
\vspace{-1.67ex}
}
\hfill
\parbox{.4\linewidth}{
\centering
\resizebox{.4\textwidth}{!}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
 & \multicolumn{3}{c}{Top-1 Accuracy(\%)} &  & \multicolumn{3}{c}{Seen-Unseen H} \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
 & AwA2 & aPY & SUN &  & AwA2 & aPY & SUN \\ \midrule
DAP~\cite{Lampert2014} & 46.1 & 33.8 & 39.9 &  & -- & 9.0 & 7.2 \\
SSE~\cite{zhang2015zero} & 61.0 & 34.0 & 51.5 &  & 14.8 & 0.4 & 4.0 \\
SJE~\cite{akata2015evaluation} & 61.9 & 35.2 & 53.7 &  & 14.4 & 6.9 & 19.8 \\
LATEM~\cite{xian2016latent} & 55.8 & 35.2 & 55.3 &  & 20.0 & 0.2 & 19.5 \\
ESZSL~\cite{romera2015embarrassingly} & 58.6 & 38.3 & 54.5 &  & 11.0 & 4.6 & 15.8 \\
ALE~\cite{akata2016label} & 62.5 & 39.7 & 58.1 &  & 23.9 & 8.7 & 26.3 \\
CONSE~\cite{norouzi2013zero} & 44.5 & 26.9 & 38.8 &  & 1.0 & -- & 11.6 \\
SYNC~\cite{changpinyo2016synthesized} & 46.6 & 23.9 & 56.3 &  & 18.0 & 13.3 & 13.4 \\
SAE~\cite{kodirov2017semantic} & 54.1 & 8.3 & 40.3 &  & 2.2 & 0.9 & 11.8 \\
DEM~\cite{zhang2016learning} & 67.1 & 35.0 & 61.9 &  & 25.1 & 19.4 & 25.6 \\
DEVISE~\cite{frome2013devise} & 59.7 & 39.8 & 56.5 &  & \textbf{27.8} & 9.2 & 20.9 \\  \hline
GAZSL~\cite{Elhoseiny_2018_CVPR} & 58.9 & 41.1 & 61.3 &  & 15.4 & 24.0 & 26.7 \\ 
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL} & \textbf{67.8} $\mathcolor{blue}{\mathbf{ ^{+8.9}}}$ & {42.1} $\mathcolor{blue}{\mathbf{ ^{+1.0}}}$ & {63.7} $\mathcolor{blue}{\mathbf{ ^{+2.4}}}$ &  & $24.6 \mathcolor{blue}{\mathbf{ ^{+9.2}}}$ & {25.7} $\mathcolor{blue}{\mathbf{ ^{+1.7}}}$ & \textbf{27.8} $\mathcolor{blue}{\mathbf{ ^{+1.1}}}$  \\
\hline \hline
FeatGen~\cite{xian2018feature} & 54.3 & 42.6 & 60.8 &  & 17.6 & 21.4 & 24.9 \\
FeatGen~\cite{xian2018feature} + \textbf{CIZSL} & $60.1\mathcolor{blue}{\mathbf{ ^{+5.8}}}$  & $43.8\mathcolor{blue}{\mathbf{ ^{+1.2}}}$ & $59.4\mathcolor{red}{\mathbf{ ^{-0.6}}}$ &  & $19.1\mathcolor{blue}{\mathbf{ ^{+1.5}}}$  & $24.0 \mathcolor{blue}{\mathbf{ ^{+2.6}}}$ & $26.5 \mathcolor{blue}{\mathbf{ ^{+1.6}}}$ \\
\midrule
cycle-(U)WGAN~\cite{felix2018multi} & 56.2 & 44.6 & 60.3 &  & 19.2 & 23.6 & 24.4 \\
cycle-(U)WGAN~\cite{felix2018multi} + \textbf{CIZSL} & $63.6 \mathcolor{blue}{\mathbf{ ^{+7.4}}}$  & \textbf{45.1} $\mathcolor{blue}{\mathbf{ ^{+0.5}}}$  & \textbf{64.2} $\mathcolor{blue}{\mathbf{ ^{+3.9}}}$   &  & $23.9 \mathcolor{blue}{\mathbf{ ^{+4.7}}}$   & \textbf{26.2} $\mathcolor{blue}{\mathbf{ ^{+2.6}}}$   & $27.6 \mathcolor{blue}{\mathbf{ ^{+3.2}}}$  \\
\bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level attributes of \textbf{AwA2}, \textbf{aPY} and \textbf{SUN} datasets.}
\label{tb:awa2_apy_sun}
}
\vspace{-2.0ex}
\end{table*}
\noindent \textbf{Ablation Study (Table~\ref{tb:nab_cub_ablation}).}  Our loss is composed of two terms shown that encourage the careful  deviation in Eq~\ref{eq_lgc}.  The first term encourages that the generated visual features from the hallucinated text $t^h$ to deceive the discriminator believing it is real, which restricts synthesized visual features to be realistic. The second term maximizes the entropy using a deviation measure.  %Our best performing entropy measure is two parameter  Shama-Mittal(SM) loss especially in the generalized SUAUC metric.
In our work, Shama-Mittal(SM) entropy  parameters $\gamma$ and $\beta$ are learnt and hence adapt the corresponding data and split mode to a matching divergence function, leading to the best results especially in the generalized SUAUC metric; see first row in Table~\ref{tb:nab_cub_ablation}. We first investigate the effect of deviating the hallucinated text by classifying it t a new class $K^s+1$, where $K^s$ is the number of the seen classes. We found the performance is significantly worse since the loss would significantly increase indecencies against seen classes and hence reduces seen knowledge transfer to unseen classes; see row 2 in  Table~\ref{tb:nab_cub_ablation}. When we remove the first term (realistic constraints), the performance degrades  especially under the generalized Seen-Unseen AUC metric because generated visual features became unrealistic; see row 3 in  Table~\ref{tb:nab_cub_ablation} (e.g., 39.2\% to 35.0\% AUC drop for CUB Easy and 11.9\%-8.2\% drop for CUB Hard). %\mohamed{comment can be better}
Alternatively, when we remove the second term (entropy), we also observe a significant drop in performance showing that both losses are complementary to each other; see row 4 in  Table~\ref{tb:nab_cub_ablation} (e.g., 39.2\% to 33.5\% AUC drop for CUB Easy and 11.9\%-10.1\% drop for CUB Hard). %\mohamed{}
In our ablation,  applying our approach without both terms (our loss) is equivalent to~\cite{Elhoseiny_2018_CVPR}, shown is the last row in Table~\ref{tb:nab_cub_ablation} as one of the least performing baselines. Note that our loss is applicable to other generative ZSL methods as we show in our state-of-the-art comparisons later in this section. 

%The last row  in Table~\ref{tb:nab_cub_ablation} shows our final best performing model as a reference which is based on Sharma-Mittal divergence.   

%This represents a basic deviation baseline but with a low-entropy in a new class, which proved to perform worse especially in the hard split\mohamed{ where the our loss is more needed.}

 

%The first row in Table~\ref{tb:nab_cub_ablation} shows our final model.

%In this ablation, we note that applying our approach without our loss is equivalent to~\cite{Elhoseiny_2018_CVPR}, which is the first row in Table~\ref{tb:nab_cub_ablation}. 

We also compare different entropy measures to encourage the deviation from the seen classes: \emph{Kullback-Leibler (KL)}, \emph{R\'enyi}~\cite{Renyi60}, \emph{Tsallis}~\cite{Tsallis88}, \emph{Bhattacharyya}~\cite{Bhattacharyya}; see rows 5-8 in Table~\ref{tb:nab_cub_ablation}. All these divergences measure are special cases of  the two parameter ($\gamma$ , $\beta$) Sharma-Mittal(SM)~\cite{sm_1976} divergence that we implemented.
%The input parameters that are needed for some divergence measures are learnt a learning weight; see Sec~\ref{sec_gen_loss} and more details in the supplementary. %SM learns the parameters $\gamma$ and $\beta$ and adapt the corresponding data and split mode to a matching divergence function, which leads to the best results especially in the generalized SUAUC metric. 
For instance, Renyi~\cite{Renyi60} and Tsallis~\cite{Tsallis88} on the other hand only learns one parameter and achieves comparable yet lower performance.  Bhattacharyya~\cite{Bhattacharyya} and KL have no learnable parameters an achieves lower performance compared to SM.%; see the first four rows in Table~\ref{tb:nab_cub_ablation}.

%Now we verify our hypothesis that maximizing entropy encourages generator to expre unseen space given hallucinated text description $t^h$ (last three rows).   
%The first term encourages that the generated visual features from the hallucinated text $t^h$ to deceive the discriminator believing it is real, which restricts synthesized visual features to be realistic. The second term maximizes the entropy using a deviation measure.  



\begin{figure}
	\centering
	\subfloat[CUB with SCS (easy) split]{\includegraphics[width= 1.6in]{img/CUB_Easy_AUC.png}} 
	\subfloat[CUB with SCE (hard) split]{\includegraphics[width= 1.6in]{img/CUB_Hard_AUC.png}}\\
    \vspace{-2mm}
	\subfloat[NAB with SCS (easy) split]{\includegraphics[width= 1.6in]{img/NAB_Easy_AUC.png}} 
	\subfloat[NAB with SCE (hard) split]{\includegraphics[width= 1.6in]{img/NAB_Hard_AUC.png}}\\
	\setlength\belowcaptionskip{-2.5ex}
	\caption{Seen-Unseen accuracy Curve with two splits: SCS(easy) and SCE(hard). Ours indicates GAZSL+ CIZSL }
    % \vspace{-1em}
	\label{fig:GZSL_Curve}
    % \vspace{-4mm}
\end{figure}
% 

% \begin{figure}
% 	\centering
% 	\subfloat[CUB with Hard Split]{\includegraphics[width= 1.6in]{figures/AUC_Hard_CUB.png}} 
% 	\subfloat[NAB with Easy Split]{\includegraphics[width= 1.6in]{figures/AUC_Easy_NABirds.png}}\\
% 	\setlength\belowcaptionskip{-2.5ex}
% 	\caption{ Seen-Unseen accuracy
% 		Curve on CUB (Hard) and NAB (Easy)}
% 	\label{fig:GZSL_Curve}
%     \vspace{-2.8mm}
% \end{figure}
\noindent \textbf{Zero-Shot Recognition and Generality on ~\cite{xian2018feature} and ~\cite{Elhoseiny_2018_CVPR}.}
Fig~\ref{fig_auklet} shows the key advantage of our CIZSL loss,  doubling the capability of [57] from 0.13 AUC to 0.27 AUC  to distinguish between two very similar birds: Parakeet Auklet (Seen class) and Crested Auklet (unseen class), in 200-way classification; see Appendix A for  details. Table~\ref{tb:nab_cub} shows state-of-the-art comparison on CUB and NAB datasets for both their SCS(easy) and SCE(hard) splits (total of four benchmarks). Our method shows a significant advantage compared to the state of the art especially in generalized Seen-Unseen AUC metric ranging from 1.0-4.5\% improvement. Fig~\ref{fig:GZSL_Curve} visualizes Seen-Unseen curves for our four benchmarks CUB (east and hard splits) and NABirds (easy and hard splits) where ours has a significant advantage compared to state-of-the-art on recognizing unseen classes; see our area under SU curve  gain in Fig~\ref{fig:GZSL_Curve}  against the runner-up GAZSL. The average relative SU-AUC improvement on the easy splits is 15.4\% and 23.56\% on the hard split. Meaning, the advantage of our loss becomes more clear as splits get harder, showing a better capability of discriminative knowledge transfer.  We show the generality of our method by embedding it with another feature generation method, FeatGen~\cite{xian2018feature}, causing a consistent improvement.  All the methods are using same text and visual representation.

\noindent \textbf{Zero-Shot Retrieval.} We investigate our model's performance for zero-shot retrieval task given the Wikipedia article of the class using mean Average Precision (mAP), the common retrieval metric. In table ~\ref{tb:Retrieval}, we report the performance of different settings: retrieving 25\%, 50\%, 100\% of the images at each class. 
We follow ~\cite{Elhoseiny_2018_CVPR} to obtain the visual center of unseen classes by generating 60 examples for the given text then computing the average. Thus, given the visual center, the aim is to retrieve images based on the nearest neighbor strategy in the visual features space. Our model is the best performing and improves the MAP (100\%) over the  runner-up (~\cite{Elhoseiny_2018_CVPR}) by 14.64\% and 9.61\% on CUB and NAB respectively. %This shows less sensitivity to the increase of number of test samples than other models because it encourages retrieving unseen classes as long as it is realistic. 
%Figure~\ref{fig:retivial} shows qualitative examples of successful and unsuccessful retrieval in CUB-SCS(easy). 
Even when the model fails to retrieve the exact unseen class, it tends to retrieve visually similar images; see qualitative examples in Appendix D. 


%This shows less sensitivity to the increase of number of test samples than other models because it encourages retrieving unseen classes as long as it is realistic.  
 %Our model shows less sensitivity to the increase of number of test samples than other models because it encourages retrieving unseen classes as long as it is realistic.  14.64\% and 9.61\%.

%We follow ~\cite{Elhoseiny_2018_CVPR} to obtain the visual center of unseen classes by generating example for the given text then computing the average. Thus, given the visual center, the aim is to retrieve images based on the nearest neighbor strategy in the visual features space. Our model shows less sensitivity to the increase of number of test samples than other models because it encourages retrieving unseen classes as long as it is realistic. Figure ~\ref{fig:retivial} shows some qualitative examples of successful and unsuccessful retrieval in CUB-SCS. Even when the model fails to retrieve the exact unseen class, it tends to retrieve visually similar images.

%The performance of our model depicts a superior retrieval performance in most of the cases and it gets  significantly better when we aim to retrieve more images of the given text (i.e., the $50\%$, and the $100\%$ case). 
 \begin{table}[]
\centering
%\resizebox{\columnwidth}{!}{%
\scalebox{0.6}
{
\begin{tabular}{cccccccc}
\hline
\multirow{2}{*}{} & \multicolumn{3}{c}{CUB} &  & \multicolumn{3}{c}{NAB} \\ \cline{2-4} \cline{6-8} 
 & 25\% & 50\% & {100\%} &  & 25\% & 50\% &{ {100\% }}\\ \hline
ESZSL \cite{romera2015embarrassingly} & 27.9 & 27.3 & 22.7 &  & 28.9 & 27.8 & 20.9 \\
ZSLNS \cite{Qiao2016} & 29.2 & 29.5 & 23.9 &  & 28.8 & 27.3 & 22.1 \\
ZSLPP \cite{Elhoseiny_2017_CVPR} & 42.3 & 42.0 & 36.3 &  & 36.9 & 35.7 & 31.3 \\
GAZSL \cite{Elhoseiny_2018_CVPR} & 49.7 & 48.3 & 40.3 &  & \textbf{41.6} & 37.8 & 31.0 \\ \hline
GAZSL \cite{Elhoseiny_2018_CVPR}+ CIZSL & \textbf{50.3}$\mathcolor{blue}{\mathbf{ ^{+0.6}}}$ & \textbf{48.9} $\mathcolor{blue}{\mathbf{ ^{+0.6}}}$ & \textbf{46.2}$\mathcolor{blue}{\mathbf{ ^{+5.9}}}$ &  & 41.0$\mathcolor{red}{\mathbf{ ^{-0.6}}}$& \textbf{40.2}$\mathcolor{blue}{\mathbf{ ^{+2.4}}}$ & \textbf{34.2}$\mathcolor{blue}{\mathbf{ ^{+3.2}}}$\\ \hline
\end{tabular}%
}
%}
\caption{Zero-Shot Retrieval using mean Average Precision(mAP) (\%) on CUB and NAB with SCS(easy) splits.}
\vspace{-3.67ex}
\label{tb:Retrieval}
\end{table}

\subsection{Attribute-based Zero-Shot Learning}
\noindent \textbf{Datasets.}  Although it is not our focus, we also investigate the performance of our model's zero-shot recognition ability using different semantic representation. We follow the GBU setting~\cite{gbu}, where images are described by their attributes instead of textual describtion deeming the problem to be relatively easier than textual-description zero-shot learning. We evaluated our approach on the following datasets: Animals with Attributes (AwA2)~\cite{lampert2009}, aPascal/aYahoo objects(aPY)~\cite{farhadi2009describing} and the SUN scene attributes dataset~\cite{patterson2012sun}. They consist of images covering a variety of categories in different scopes: animals, objects and scenes respectively. AwA contains attribute-labelled classes but aPY and SUN datasets have their attribute signature calculated as the average of the instances belonging to each class. 

\noindent \textbf{Zero-Shot Recognition.} %To show the generality of our method, we also perform Zero-Shot recognition on this setting.
On AwA2, APY, and SUN datasets, we show in Table~\ref{tb:awa2_apy_sun} that our CIZSL loss improves three generative zero-shot learning models including GAZSL~\cite{Elhoseiny_2018_CVPR},  FeatGen~\cite{xian2018feature},  and  cycle-(U)WGAN~\cite{felix2018multi}.
% (FeatGen~\cite{xian2018feature},  cycle-(U)WGAN~\cite{felix2018multi}, and GAZSL~\cite{Elhoseiny_2018_CVPR})
The table also shows our comparison to the state-of-the-art where we mostly obtain a superior performance. Even when obtaining a slightly lower score than state-of-the-art on AWA2, our loss adds a 9.2\% Seen-Unseen H absolute improvement to the non-creative GAZSL~\cite{Elhoseiny_2018_CVPR}. We also evaluated our loss on \emph{CUB-T1(Attributes) benchmark~\cite{gbu}}, where the Seen-Unseen H for  GAZSL~\cite{Elhoseiny_2018_CVPR}] and GAZSL~\cite{Elhoseiny_2018_CVPR}+CIZSL are 55.8 and  57.4, respectively. 
% : ( Seen-Unseen H 55.8), 
%  ( Seen-Unseen H  57.4). 

% \subsection{Discussion}

% We hypothesized that our method is better in generalization than standard generative ZSL approaches at L51-151 in the main paper. We conduct an additional experiment to verify this claim by plotting the Seen-Unseen curves for only Parakeet Auklet among the seen classes and Crested Auklet among the unseen classes. We note that the prediction space (T) still includes the 200 CUB species (see Fig~\ref{fig_auklet}), but with a focus on analyzing these two categories.  The AUC for the baseline GAZSL is 0.139 and for our CIZSL (GAZSL + our loss) is 0.271 $\approx$ 100\% relative improvement for discriminating these two classes. This demonstrates how the confusion between those two classes is drastically reduced by using our loss, especially for the unseen Crested Auklet (x-axis).
% %  We validate our hypothesis about parakeet Auklet vs Crested Auklet in L51-151 in the paper in our experiments but plotting the Seen Unseen curves for only Parakeet Auklet among the  seen classes and Crested Auklet among the unseen classes. Note that the prediction space is still the 200 CUB species but we focus on analyzing these two categories to quantify how the confusion between these two classes is significantly reduced with our loss and especially for the unseen unseen Crested Auklet (the x=axis). 
% \begin{figure}[th!]
% \vspace{-7mm}
% 	\centering
%   \includegraphics[width=0.5\textwidth,height=7.1cm]{figures/ParakeetAuklet_vs_CrestedAukletAUC.png}
%   \vspace{-2mm}
% 	\caption{Seen Unseen Curve for Parakeet Auklet (Seen) on the y-axis versus Crested Auklet (unseen) on the x-axis for GAZSL  and CIZSL (GAZSL+our loss) }
% % 		\vspace{-3mm}
% 	\label{fig_auklet}
% \end{figure}
% \vspace{-2mm}
% \newpage
% In this section, we investigate the following aspects of the ZSL problem. First, the effect of the creativity based approach on description-based semantic representation (i.e. body of text describing a class). Second, the effect of our prior on the attribute-based semantic representation (i.e., collection of semantic characteristics uniquely describe classes). Third, examine a generic class of entropic measures, to select the most suitable one for our loss. Finally, if our loss proved to help in zero-shot recognition, we also need to explore its abstraction by conducting zero-shot retrieval experiments. We note that we consider description-based ZLS as our major experimental protocol since it is a more generic and harder problem than the attribute-based ZLS. That's why we use it to perform the ablation study and the ZLS retrieval experiments.

% We investigate the following aspects of ZSL problem: Zero Shot Recognition for Class-level Text description as well as attribute-based

% We performed extensive experiments on four splits for Wikipedia-based zero-shot learning that we focus on. Near the end, we also evaluated our approach for attribute-based zero-shot learning on three dataset to show the advantage of our approach. 
% we evaluate the performance of our approach on two semantic settings: class-level text description and attribute-based text description. Since the class-level description is a more generic and harder problem to solve, we use it to perform the ablation study and Zero-Shot retrieval. For both settings, we compare our approach with state-of-the-art Zero-Shot Recognition methods.

 %In~\cite{Elhoseiny_2017_CVPR}, a new merge of the classes in NAB was proposed to constitute 404 classes instead of 1011. Specifically, it targeted merging classes of the same species but merely differ in gender such as ``American Kestrel (Female, immature)" and ``American Kestrel (Adult male)" since there is one Wikipedia text for both genders. 
    %==> Mentioned in the approach
%\noindent \textbf{Image Representation} Zhang \emph{et al.}~\cite{zhang2016spda} showed that fine-grained recognition of bird species can be improved by detecting objects parts and learning a part-based learning representations on top.They named  their network Visual Part Detector/Encoder network (VPDE-net). Following~\cite{zhang2016spda}, we adopt fast-RCNN framework~\cite{girshick2015fast} with VGG16 backbone architecture~\cite{simonyan2014very} to detect semantic parts of birds(e.g., head, leg, wing, etc.). Concretely, the input image is fed forward to earlier VGG16 convolutional layer where Nearest neighbor proposals, introduced by  by~\cite{zhang2016spda}, are generated. The proposals are then fed to a ${p+1}$-way part classifier and a bounding box regressor, where $p$ is the number of parts and the extra class is background. Each part $p$ is considered detected if there exist at least a proposal classified to part $p$ with a confidence bigger than a threshold. If detected, it is then assigned to the region of the highest confidence. The regions corresponding to detected parts are then fed to a visual encoding subetwork that finally produce a $512D$ feature vector for every detected part. We visually represent the images by the concatenation of the feature vectors of each semantic part (i.e., $p*512D$).

% As we argued earlier, this term makes the deviation from seen classes encouraged by the fourth term  careful not to fall in the unrealistic range illustrated Fig~\ref{fig:intro}. Alternatively, when we remove the max-entropy term (the fifth Eq~\ref{eq:gen}), we also observe a significant drop in performance showing that both losses are complementary to each other. We have a similar observation when we remove both terms which is equivalent to~\cite{Elhoseiny_2018_CVPR}; see the last four tows in Table~\ref{tb:nab_cub_ablation}.


% We start by invistigate the effect of classifying the hallucinated text with a lower entropy as a new class $N+1$ , where $N$ is the number of training classes. Evidently, having a lower entropy as a new class (first row) performs poorly relative to enforcing a high entropy classification over all training classes (the rest of the table), which further supports our hypothesis.
% As a final baseline, we also 


% \noindent \mohamed{we may remove Results Overview.}
%  \textbf{Results Overview.}
% Our experiments explore the SCS(easy) and SCE(hard) splits on the both CUB and NABirds  datasets. Our main objective is to illustrate the effectiveness of modeling zero-shot learning with creativity inspiration perspective. We performed ablation studies to show that the proposed losses and component are necessary to achieve the desired performance.  We also explored different entropy losses to model the deviation from the seen classes and showed that a learnable entropy measure leads to the best performance.  


% \noindent \textbf{Comparison to the State-of-The art.} We compared our method with the following state-of-the-art baselines:  GZSL~\cite{Elhoseiny_2018_CVPR}, ZSLPP~\cite{Elhoseiny_2017_CVPR}, 
% ZSLNS~\cite{Qiao2016}, ESZSL~\cite{romera2015embarrassingly}, SJE~\cite{akata2015evaluation}, WAC~\cite{elhoseiny2013write}, and SynC~\cite{changpinyo2016synthesized}. 
% In our experiments, all these methods uses the same aforementioned visual and text representations. 


% ====================================== First Draft ========================================= %



%\subsection{Experimental Setting}


%Both datasets are used for fine-grained classification since their classes are quite similar with a significant feature overlap.

% This new merge targeted joining subtle division of classes. 


%The reason was due to the lack of available textual description separating species based on gender that could be found on Wikipedia. % In the problem of zero-shot learning, the target is to classify a visual representation given only textual description, without seeing any visual representation of the same class before.
% \noindent \textbf{Textual Representation:}
% We use the raw Wikipedia articles collected by~\cite{Elhoseiny_2017_CVPR} for both benchmark datasets.
% Text articles are first tokenized into
% words, the stop words are removed, and porter stemmor~\cite{Porter} is applied to reduce inflected words to their word stem.  Then, Term
% Frequency-Inverse Document Frequency(TF-IDF) feature
% vector~\cite{salton1988term} is extracted. The dimensionalities of TF-IDF features for CUB and
% NAB are 7551 and 13217.
% \noindent \textbf{Visual Features:}
% We extract the visual features from the activations of the part-based FC layer of VPDE-net. All input images are resized to $224 \times 224$ and fed into the VPDE-net. There are seven semantic parts in CUB dataset: ``head", ``back", ``belly", ``breast", ``leg", ``wing", ``tail". NAB dataset contains the same semantic parts except for ``leg". For each part, a 512-dimensional feature vector is extracted. Concatenating those part-based features in order, we obtain the visual representation of the image. The dimensionalities of visual features for CUB and NAB are 3583 and 3072 respectively. 
% [Textual representation]
% [Visual representation]
%Upon our introduction of the $L_e$ loss, we need to account for the weight of such loss in the joint loss contributing to the training.
%Therefore,


% \subsection{Seen Classes Deviation Loss}

% \mypar{Multi-classCross Entropy loss}
% %-----------------------------------------
% We propose to use as $\mathcal{L}_{G\mbox{ \scriptsize{creativity}}}$ the Multi-class Cross Entropy (MCE) loss between the class prediction of the discriminator and the uniform distribution. The goal is for the generator to make the generations hard to classify by the discriminator.
% \begin{equation}
% \mathcal{L}_{\mbox{\scriptsize{MCE}}} = -\sum_{i} \sum_{k=1}^K \frac{1}{K} \log \left(\frac{e^{D_{b,k}(G(z_i))}}{\sum_{q=1}^K e^{D_{b,q}(G(z_i))}}
% \right) =-\sum_{i} \sum_{k=1}^K \frac{1}{K}\log (\hat{D_i}),
% \label{eq_MCE}
% \end{equation}

% %We denote this criterion as CAN(H), for Creative Adversarial Network with Holistic loss.
% where \ccc{$\hat{D_i}$ is the softmax of $D_b(G(z_i))$}. %= \frac{e^{D_{b,\hat{c}_i}(G(z_i))}}{\sum_{k=1}^K e^{D_{b,k}(G(z_i))}}$.
% In contrast to the CAN loss that treats every classification independently, the MCE loss should better exploit the class information in a global way. \omitme{ Both MCE and
% sum of binary cross entropies losses encourage deviation from existing categories (shapes/textures here). Since the generator is
% trained to output images that are not associated with
% any label, the CAN loss can not contrast against negatives
% and hence merely look at each dimension interdependently
% encouraging it to get close to $\frac{1}{K}$.} \omitme{ ccc I removed the paragraph because: 1st sentense: redundant; 2nd "are not associated with any label" : true for MCE too. "can not contrast against negatives" : to rephrase: what are negative here?}

% Our MCE loss is in fact equivalent to a Kullback-Leibler (KL) loss between a uniform distribution and the softmax output, since the entropy term of the uniform distribution is constant\me{; see derivation in Eq.~\ref{eq_KL}.}

% \begin{equation}
%  \me{ \mathcal{L}_{\mbox{\scriptsize{KL}}} = \sum_{i,k}  \frac{1}{K} \log (\frac{1}{K \hat{D_i}}) = \sum_{i,k}  \frac{1}{K} \log (\frac{1}{K})- \sum_{i,k} \frac{1}{K} \log (\hat{D_i}) 	\propto - \sum_{i,k} \frac{1}{K} \log (\hat{D_i}) = \mathcal{L}_{\mbox{\scriptsize{MCE}}}}
% \label{eq_KL}
% \end{equation}

% It is more meaningful
% conceptually to define the deviation over the joint distribution
% over the categories which is what we modeled by
% the KL divergences between the softmax probabilities and
% the prior (defined as uniform in our case), as it also opens the door to study other
% divergence measures. Finally, the MCE loss requires less compute comparing to CAN.



% \begin{figure}[htb]
%   \begin{center}
% \includegraphics[width=0.16\linewidth]{highest_NN_dist_0465copy.png}
% \includegraphics[width=0.16\linewidth]{highest_NN_dist_0484copy.png}
% \includegraphics[width=0.16\linewidth]{highest_shape_entropy_0019copy.png}
% \includegraphics[width=0.16\linewidth]{highest_NN_dist_0485copy.png}
% \includegraphics[width=0.16\linewidth]{lowest_shape_entropy_0109copy.png}
% \includegraphics[width=0.16\linewidth]{low_shape_high_NN_dist_0778copy.png}
%   \end{center}
%   \caption{Some generations from a DCGAN
%     with MCE creativity loss applied on texture (Model GAN MCE tex).}
%   \label{fig:best}
% \end{figure}

% %-------------------------------------------
% \mypar{Generalized Sharma-Mittal Divergence}
% We further generalize the expression of the creativity term to a broader family of divergences, unlocking new way of enforcing deviation from existing shapes and textures.
% \cite{IsSM07} studied an entropy measure called Sharma-Mittal \omitme{on thermostatics in 2007,}which was originally introduced by \cite{SM75}. Given two parameters ($\alpha$ and $\beta$), %SM  relative entropy (mutual information) generalizes each of the R\'enyi, Tsallis and KL mutual information divergences.
%  the Sharma-Mittal (SM) divergence $SM_{\alpha, \beta}(p\|q)$,  between two distributions $p$ and $q$ is defined $\forall \alpha >0,~\alpha \neq 1,~\beta \neq 1$ as %~\citep{SM75}
% \begin{equation}
% SM(\alpha, \beta)(p || q) = \frac{1}{\beta-1} \left[ \sum_i (p_i^{1-\alpha} {q_i}^{\alpha})^\frac{1-\beta}{1-\alpha} -1\right]
% \label{eq:smgen}
% \end{equation}
% It was shown in~~\citep{IsSM07} that most of the widely used divergence measures are special cases of SM divergence. For instance, each of the R\'enyi, Tsallis and Kullback-Leibler (KL) divergences can be defined as limiting cases of SM divergence as follows:
% \begin{equation}
% \small
% \begin{split}
% R_{\alpha}(p\|q) = &\lim_{\beta \to 1} {SM_{\alpha, \beta}(p\|q) }  = \frac{1}{\alpha-1} \ln (\sum_i {p_i^\alpha q_i^{1-\alpha} } )),  \\
% T_{\alpha}(p\|q) = &\lim_{\beta \to \alpha} {SM_{\alpha, \beta}(p\|q) }= \frac{1}{\alpha-1} (\sum_i {p_i^\alpha q_i^{1-\alpha} } ) -1),  \\
% KL(p\|q) = & \lim_{\beta \to 1, \alpha \to 1} {SM_{\alpha, \beta}(p\|q) } = \sum_i{p_i \ln ( \frac{p_i}{q_i}}).
% \end{split}
% \omitme{\begin{split}
% R_{\alpha}(p\|q) = &\lim_{\beta \to 1} {SM_{\alpha, \beta}(p\|q) }  = \frac{1}{\alpha-1} \ln (\int_{-\infty}^{\infty}{p(t)^\alpha q(t)^{1-\alpha} dt} )),  \\
% T_{\alpha}(p\|q) = &{SM_{\alpha, \alpha}(p\|q) }= \frac{1}{\alpha-1} (\int_{-\infty}^{\infty}{p(t)^\alpha q(t)^{1-\alpha} dt} ) -1),  \\
% KL(p\|q) = & \lim_{\beta \to 1, \alpha \to 1} {SM_{\alpha, \beta}(p\|q) } = \int_{-\infty}^{\infty}{p(t) \ln ( \frac{p(t)}{q(t)} dt})
% \end{split}}
% \label{eqdef}
% \end{equation}
% \ccc{In particular, the } Bhattacharyya divergence ~\citep{bhatt67}, denoted by $B(p\|q)$   is a limit case of SM and R\'enyi divergences as follows as $\beta \to 1, \alpha \to 0.5$
% \begin{equation*}
% \small

% \begin{split}
% B(p\|q)& = 2 \lim_{\beta \to 1, \alpha \to 0.5}  SM_{\alpha,\beta}(p\|q)  = - \ln \Big( \sum_i p_i^{0.5} q_i^{0.5} \Big).
% \end{split}
% \end{equation*}
% Since the notion of creativity in our work is grounded to maximizing the deviation from existing shapes and textures through KL divergence in Eq~\ref{eq_KL}, we can  generalize our MCE creativity loss by minimizing  Sharma Mittal (SM) divergence   between a uniform distribution and the softmax output $\hat{D}$ as follows
% \begin{equation}
% \begin{split}
% \mathcal{L}_{SM} = SM(\alpha,\beta)( \hat{D} || u) =
% SM(\alpha, \beta)(\hat{D} || u) = \frac{1}{\beta-1} \sum_i (\frac{1}{K}^{1-\alpha} {\hat{D_i}}^{\alpha})^\frac{1-\beta}{1-\alpha} -1
% \end{split}
% \label{eq_sm}
% \end{equation}
% Note that the MCE loss in Eq~\ref{eq_KL} is a special case of the generalized SM loss where $\alpha \to 1$ and $\beta \to 1$ (i.e., KL divergence). Similarly, Tsallis , and Renyi, and Bhattacharyya losses are  special cases of SM loss where $\alpha = \beta$, $\beta \to 1$ and $\alpha \to 0.5$ and $\beta \to 1$. \me{We explored various parameters but we found both KL and  Bhattacharyya losses work the best and hence we focus on them in our experiments.} \ccc{We denote models trained with these losses by MCE and SM respectively.} %We explore some of these cases in our work.

  
%For each of those methods, MCZL and ZSLPP uses the semantic parts of birds for visual representations of images. In particular, MCZL uses the annotations of the parts as strong supervision used to extract a CNN representation of each semantic part at the inference time. 
%Hence, each trial generates an $(x,y)$ co-ordinate where $x$ and $y$ are the unseen and seen test accuracy. that forms the seen-unseen curve. 
%for each value which generates to draw Seen-Unseen Curve(SUC) and% Visual features of each class are averaged to obtain visual .



%several variations of creativity loss. %Hence, the most relevant approach to our approach will be ~\cite{Elhoseiny_2018_CVPR}. This approach presents the standard adversarial training with no further modifications. Our approach adopt a similar training paradigm by adversarially learning to generate visual features from text description, but it further synthesizes unseen classes and generalize the class training to enable generalization at the inference time to unseen classes. 







% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccccccccccccccc@{}}
% \toprule
% Metric & \multicolumn{7}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{7}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-8} \cmidrule(l){10-16} 
% Dataset & \multicolumn{2}{c}{CUB} & \multirow{2}{*}{APY} & \multirow{2}{*}{AWA2} & \multirow{2}{*}{SUN} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multirow{2}{*}{APY} & \multirow{2}{*}{AWA2} & \multirow{2}{*}{SUN} & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(lr){7-8} \cmidrule(lr){10-11} \cmidrule(l){15-16} 
% Split-Mode & SCS & SCE &  &  &  & SCS & SCE &  & SCS & SCE &  &  &  & SCS & SCE \\ \midrule

% WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 & -- & -- & -- & -- & -- &  & 23.9 & 4.9 & -- & -- & -- & 23.5 & -- \\
% WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 & -- & -- & -- & 11.4 & 6.0 &  & 14.7 & 4.4 & -- & -- & -- & 9.3 & 2.3 \\
% ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 & 58.6 & 38.3 & 54.5 & 24.3 & 6.3 &  & 18.5 & 4.5 & 11.0 & 4.6 & 15.8 & 9.2 & 2.9 \\
% ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & -- & -- & -- & 24.5 & 6.8 &  & 14.7 & 4.4 & -- & -- & -- & 9.3 & 2.3 \\
% SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & -- & -- & -- & 18.4 & 3.8 &  & 13.1 & 4.0 & -- & -- & -- & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 & -- & -- & -- & -- & -- &  & 1.7 & 1.0 & -- & -- & -- & 0.1 & --\\
% CONSE \cite{norouzi2013zero} & -- & -- & 44.5 & 26.9 & 38.8 & -- & -- &  & -- & -- & 1.0 & -- & 11.6 & -- & -- \\
% SSE \cite{zhang2015zero} & -- & -- & 61.0 & 34.0 & 51.5 & -- & -- &  & -- & -- & 14.8 & 0.4 & 4.0 & -- & -- \\
% LATEM \cite{xian2016latent} & -- & -- & 55.8 & 35.2 & 55.3 & -- & -- &  & -- & -- & 20.0 & 0.2 & 19.5 & -- & -- \\
% SAE \cite{kodirov2017semantic} & -- & -- & 54.1 & 8.3 & 40.3 & -- & -- &  & -- & -- & 2.2 & 0.9 & 11.8 & -- & -- \\
% ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2  &9.7 & -- & -- & -- & 30.3 & 8.1 &  & 30.4 & 6.1 & -- & -- & -- & 12.6 & 3.5 \\
% GAZSL \cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 58.9 & 41.1 & 61.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 15.4 & 24.0 & 26.7 & 20.4 & 5.8 \\    \midrule
% Ours &  \textbf{44.61} & \textbf{14.38} &  &  &  & \textbf{36.53} & \textbf{9.229} &  & \textbf{39.15} & \textbf{11.94} &  &  &  & \textbf{24.45} & \textbf{6.38} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation Performance of \textbf{CUB} and \textbf{NAB} datasets with two split settings.}
% \label{tb:nab_cub}
% \end{table*}

% \begin{table}[]
% \centering
% \resizebox{.48\textwidth}{!}{%
% \begin{tabular}{@{}cccccccc@{}}
% \toprule
%  & \multicolumn{3}{c}{Top-1 Accuracy(\%)} &  & \multicolumn{3}{c}{Seen-Unseen AUC} \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
%  & AwA2 & aPY & SUN &  & AwA2 & aPY & SUN \\ \midrule
% DAP~\cite{Lampert2014} & 46.1 & 33.8 & 39.9 &  & -- & 9.0 & 7.2 \\
% CONSE & 44.5 & 26.9 & 38.8 &  & 1.0 & --- & 11.6 \\
% SSE & 61.0 & 34.0 & 51.5 &  & 14.8 & 0.4 & 4.0 \\
% DEVISE~\cite{frome2013devise} & 59.7 & 39.8 & 56.5 &  & \textbf{27.8} & 9.2 & 20.9 \\
% SJE~\cite{akata2015evaluation} & 61.9 & 35.2 & 53.7 &  & 14.4 & 6.9 & 19.8 \\
% LATEM & 55.8 & 35.2 & 55.3 &  & 20.0 & 0.2 & 19.5 \\
% ESZSL~\cite{romera2015embarrassingly} & 58.6 & 38.3 & 54.5 &  & 11.0 & 4.6 & 15.8 \\
% ALE~\cite{akata2016label} & 62.5 & 39.7 & 58.1 &  & 23.9 & 8.7 & 26.3 \\
% SYNC~\cite{changpinyo2016synthesized} & 46.6 & 23.9 & 56.3 &  & 18.0 & 13.3 & 13.4 \\
% SAE & 54.1 & 8.3 & 40.3 &  & 2.2 & 0.9 & 11.8 \\
% DEM~\cite{zhang2016learning} & \textbf{67.1} & 35.0 & 61.9 &  & 25.1 & 19.4 & 25.6 \\
% GAZSL~\cite{Elhoseiny_2018_CVPR} & 58.9 & 41.1 & 61.3 &  & 15.4 & 24.0 & 26.7 \\ \midrule
% Ours & 64.47 & \textbf{42.02} & \textbf{63.7} &  & 20.4 & \textbf{25.7} & \textbf{27.8} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation Performance of \textbf{AwA2}, \textbf{aPY} and \textbf{SUN} datasets.}
% \label{tb:awa2_apy_sun}
% \end{table}




% \begin{table}[]
% \centering
% \resizebox{.48\textwidth}{!}{%
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
% Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
% Split-Mode & SCS & SCE & SCS & SCE &  & SCS & SCE & SCS & SCE \\ \midrule
% WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 & -- & -- &  & 23.9 & 4.9 & 23.5 & -- \\
% WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 & 11.4 & 6.0 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
% ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 & 24.3 & 6.3 &  & 18.5 & 4.5 & 9.2 & 2.9 \\
% ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & 24.5 & 6.8 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
% SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & 18.4 & 3.8 &  & 13.1 & 4.0 & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 & -- & -- &  & 1.7 & 1.0 & 0.1 & --\\
% ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2 & 9.7 &30.3 & 8.1 &  & 30.4 & 6.1 & 12.6 & 3.5 \\
% GAZSL \cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\    \midrule
% Ours &  \textbf{44.61} & \textbf{14.38} & \textbf{36.53} & \textbf{9.229} &  & \textbf{39.15} & \textbf{11.94} & \textbf{24.45} & \textbf{6.38} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation Performance of \textbf{CUB} and \textbf{NAB} datasets with two split settings.}
% \label{tb:nab_cub}
% \end{table}


%w/o $D(G(z_c, T_c))$
%$D(G(z_c, T_c))$




% \begin{table}[]
% \centering
% \resizebox{.48\textwidth}{!}{%
% \begin{tabular}{@{}cccccccccccc@{}}
% \toprule
% Metric & \multicolumn{5}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{5}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-6} \cmidrule(l){8-12} 
% Dataset & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\
% Split-Mode & SCS & SCE &  & SCS & SCE &  & SCS & SCE &  & SCS & SCE \\ \midrule
% WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 &  & -- & -- &  & 23.9 & 4.9 &  & 23.5 & -- \\
% WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 &  & 11.4 & 6.0 &  & 14.7 & 4.4 &   & 9.3 & 2.3 \\
% ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 &  & 24.3 & 6.3 &  & 18.5 & 4.5 &  & 9.2 & 2.9 \\
% ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & & 24.5 & 6.8 &  & 14.7 & 4.4 & & 9.3 & 2.3 \\
% SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & & 18.4 & 3.8 &  & 13.1 & 4.0 & & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 &   & -- & -- &  & 1.7 & 1.0 &  & 0.1 & --\\
% ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2  &9.7 & & 30.3 & 8.1 &  & 30.4 & 6.1 &  & 12.6 & 3.5 \\
% GAZSL \cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 &  & 35.6 & 8.6 &  & 35.4 & 8.7 &  & 20.4 & 5.8 \\    \midrule
% Ours &  \textbf{44.61} & \textbf{14.38} &  & \textbf{36.53} & \textbf{9.229} &  & \textbf{39.15} & \textbf{11.94} &  & \textbf{24.45} & \textbf{6.38} \\ \bottomrule
% \end{tabular}%
% }
% \caption{Evaluation Performance of \textbf{CUB} and \textbf{NAB} datasets with two split settings.}
% \label{tb:nab_cub}
% \end{table}






% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccccccccccccccc@{}}
% \toprule
% Metric & \multicolumn{7}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{7}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-8} \cmidrule(l){10-16} 
% Dataset & \multicolumn{2}{c}{CUB} & \multirow{2}{*}{APY} & \multirow{2}{*}{AWA2} & \multirow{2}{*}{SUN} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multirow{2}{*}{APY} & \multirow{2}{*}{AWA2} & \multirow{2}{*}{SUN} & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(lr){7-8} \cmidrule(lr){10-11} \cmidrule(l){15-16} 
% Split-Mode & SCS & SCE &  &  &  & SCS & SCE &  & SCS & SCE &  &  &  & SCS & SCE \\ \midrule
%  MCZSL \cite{akata2016multi} & 34.7 & -- &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% WAC-Linear \cite{elhoseiny2013write} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% WAC-Kernel \cite{elhoseiny2016write}  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% ESZSL \cite{romera2015embarrassingly} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% SJE \cite{akata2015evaluation} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% ZSLNS \cite{Qiao2016} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
%  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ 
% SynC$_{fast}$ \cite{changpinyo2016synthesized} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% ZSLPP \cite{Elhoseiny_2017_CVPR} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
% GAZSL \cite{Elhoseiny_2018_CVPR} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\    \midrule
% Ours & \textbf{44.6} & \textbf{14.4} &  &  &  & \textbf{36.6} & \textbf{9.3} &  &  \textbf{39.2} & \textbf{12.0}  &  &  &  & \textbf{24.5} & \textbf{6.4} &  &  \\ \bottomrule
% \end{tabular}%
% }
% \caption{My caption}
% \label{my-label}
% \end{table*}
% \begin{table}[]
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
%  & SCS & SCE &  & SCS & SCE \\ \midrule
%  MCZSL \cite{akata2016multi}   	&  34.7 & -- &   &--&--\\
% WAC-Linear \cite{elhoseiny2013write} &  27.0  &   5.0&   &--&--\\	%\hline
% WAC-Kernel \cite{elhoseiny2016write}    	&  33.5    & 7.7 &  & 11.4 &6.0\\	%\hline
% ESZSL \cite{romera2015embarrassingly}     	&  28.5   &7.4 &  &24.3&6.3\\	%\hline
% SJE \cite{akata2015evaluation}  & 29.9 & --& &  --&--\\
% ZSLNS \cite{Qiao2016}  	&  29.1   &7.3 & &  24.5&6.8\\	%\hline
% SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 &&  18.4&3.8\\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 &  5.9 & &  --&--\\
% ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2  &9.7 & & 30.3 & 8.1 \\
% GAZSL \cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 &  & 35.6 & 8.6 \\ \midrule
% CGAZSL & \textbf{44.61} & \textbf{14.38} &  & \textbf{36.53} & \textbf{9.229} \\ \bottomrule
% \end{tabular}
% \caption{Top-1 accuracy (\%) on \textbf{CUB} and \textbf{NAB} datasets with two split settings.}
% \label{tb:top_1_accuracy}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
%  & SCS & SCE &  & SCS & SCE \\ \midrule
% ESZSL \cite{romera2015embarrassingly}     	&  18.5   &4.5 &  &9.2&2.9\\	%\hline
% ZSLNS \cite{Qiao2016}  	&  14.7   &4.4 & &  9.3&2.3\\	%\hline
% WAC-Kernel \cite{elhoseiny2016write}  	&  22.5  &   7.0&   &0.7&2.3\\	%\hline
% WAC-Linear \cite{elhoseiny2013write}    	&  23.9 & 4.9 &  & 23.5 &--\\	%\hline
% SynC$_{fast}$ \cite{changpinyo2016synthesized} & 13.1 & 4.0 &&  2.7&3.5\\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 1.7 &  1.0 & &  0.1&--\\
% ZSLPP \cite{Elhoseiny_2017_CVPR}    	&  30.4  &6.1 & &  12.6&3.5\\
% GAZSL \cite{Elhoseiny_2018_CVPR}& 35.4 & 8.7 &  & 20.4 & 5.8 \\ \midrule
% CGAZSL & \textbf{39.15} & \textbf{11.94} &  & \textbf{24.45} & \textbf{6.38} \\ \bottomrule
% \end{tabular}
% \caption{Seen-Unseen Area Under Curve (\%) on \textbf{CUB} and \textbf{NAB} datasets with two split settings.}
% \label{tb:generalized_accuracy}
% \end{table}
%We conduct an ablation study on different divergence measure that we discussed in Sec~\ref{sec_gen_loss} including .
%The purpose of such experiments is to find the most effective divergence that can be used that boosts the performance on the test benchmark.
%We note that it was shown by ~\cite{sm_tsallis} that most of the widely used divergence measures are special cases of SM divergence as elaborated in the approach section. 
%The basic baseline that we compare to is performing Zero-Shot Learning with standard adversarial loss, similar to ~\cite{Elhoseiny_2018_CVPR} in GAZSL.


%Sharma-Mittal~\cite{sm_1976} divergence which is relatively less known; see Eq~\ref{le_eq}. It was shown in~\cite{IsSM07},  that other divergence measures are special case of Sharma-Mittal divergence by setting its two parameters $\gamma$ and $\beta$. It is equivalent to  \emph{R\'enyi}~\cite{Renyi60} when $\beta \to 1$ (single-parameter), \emph{Tsallis} divergence~\cite{Tsallis88} when $\gamma=\beta$ (single-parameter), Bhattacharyya divergence when$\beta \to 0.5$ and $\gamma \to 0.5$,  and \emph{Kullback-Leibler (KL)} divergence when $\beta \to 1$ and $\gamma \to 1$ (no-parameter). So, when we implement Sharma-Mittal loss, we can also  minimize all the special-case divergence measures; see more details in the supplementary. In our work, when we train with Sharma-Mittal loss, we also learn $\gamma$ and $\beta$.  
%This baseline is correspondent of our method with a creative weight loss equals to zero.
%By applying various divergence measures, we construct 

%MCZSL~\cite{akata2016multi},%We directly copy the highest scores for non-attribute settings reported in~\cite{Elhoseiny_2018_CVPR}.



%in diverging the generated features from the seen classes. 
%That might lend to one of two outcomes. Either generalizing the generated features to unseen classes, or deeming the generated features to be unrealistic. That's why we also attempt to deceive the discriminator by thinking the hallucinated text is real by applying a generative-like loss. This loss forces visual features to still be realistic,

%however being generalized by the entropy constrain. Thus, we obtain a final ablation where we conduct an experiment showing the effect of the generative-like loss as opposed to only the divergence. Evidently, when optimizing only for generative-like loss it obtains comparable results to the GAZSL ~\cite{Elhoseiny_2018_CVPR}. This is because method learns to generate features similar to seen classes, but it does not generalize well to unseen classes. However, when only maximizing the entropy of the obtained features over all the seen classes, visual features tend to be non-realistic and causes a significant degradation in the results. Mixing both losses (Sharma-Mettal and generative-like loss) finally obtains the best set of results using the two evaluation metrics: top-1\% accuracy and the seen-unseen Area-Under-Curve. We note that the upper half of both tables are using both losses but with different divergence metrics: Bachatera, Renyi, KL, Tsallis.





% \begin{table}[]
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
%  & SCS & SCE &  & SCS & SCE \\ \midrule
% GAZSL \cite{Elhoseiny_2018_CVPR}	&  43.7 & 10.3 &  & 35.6 & 8.6 \\
% Bachatera-Divergence	&  44.12  &  13.71&   &35.88 & 8.94\\
% Renyi-Divergence &  44.06 & 13.29 &  & 35.78 & 8.848\\	
% KL-Divergence	&  44.46 & 14.15 &  & 36.31 & 8.93\\	
% Tsallis-Divergence	&  44.13 & 13.84 & & \textbf{36.74} & 8.95 \\   \midrule
% SM-Entropy & \textbf{44.61} & \textbf{14.38} &  & 36.53 & \textbf{9.229} \\
% w/o $D(G(z_c, T_c))$ & 41.73 & 11.2 &  & 33.4 & 8.1 \\
% $D(G(z_c, T_c))$ & 43.4 & 10.1 &  & 35.2 & 8.3 \\\bottomrule
% \end{tabular}
% \caption{Ablation Study of Adversarial training to Zero-Shot Learning with respect to Top 1 Accuracy (\%).}
% \label{tb:ablation study_top_1}
% \end{table}  





	%\subfloat[]{\includegraphics[width= 1.2in]{motion2-crop.pdf}} \quad
	%\subfloat[]{\includegraphics[width= 1.2in]{motion3-crop.pdf}}
% \begin{table}[]
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
%  & SCS & SCE &  & SCS & SCE \\ \midrule
% GAZSL \cite{Elhoseiny_2018_CVPR}	&  35.4 & 8.7 &  & 20.4 & 5.8 \\
% Tsallis-Divergence	&  38.95 &11.33 & & 24.45 & 6.34 \\	
% Bachatera-Divergence	&  38.85  &  10.27&   &24.33 & 6.17\\
% Renyi-Divergence &  38.64 & 10.28 &  & 23.71 &6.34\\	
% KL-Divergence	&  38.89 & 11.59 &  & 24.26 & 6.27\\ \midrule
% SM-Entropy + D & \textbf{39.15} & \textbf{11.94} &  & \textbf{24.45} & \textbf{6.38} \\ 
% w/o $D(G(z_c, T_c))$ & 37.43 & 10.12 &  & 21.31 & 5.4 \\
% $D(G(z_c, T_c))$ & 35.0 & 8.2 &  & 20.1 & 5.4 \\\bottomrule
% \end{tabular}
% \caption{Ablation Study of Adversarial ` to Zero-Shot Learning with respect to seen-unseen Area Under Curve(\%).}
% \label{tb:ablation study_generalized}
% \end{table}  

% \begin{table}[]
% \centering
% \begin{tabular}{@{}cccccc@{}}
% \toprule
% \multirow{2}{*}{} & \multicolumn{2}{c}{CUB} &  & \multicolumn{2}{c}{NAB} \\ \cmidrule(lr){2-3} \cmidrule(l){5-6} 
%  & SCS & SCE &  & SCS & SCE \\ \midrule
% GAZSL \cite{Elhoseiny_2018_CVPR}	&  43.7 & 10.3 &  & 35.6 & 8.6 \\
% Bachatera-Divergence	&  44.12  &  13.71&   &35.88 & 8.94\\
% Renyi-Divergence &  44.06 & 13.29 &  & 35.78 & 8.848\\	
% KL-Divergence	&  44.46 & 14.15 &  & 36.31 & 8.93\\	
% Tsallis-Divergence	&  44.13 & 13.84 & & \textbf{36.74} & 8.95 \\   \midrule
% SM-Entropy & \textbf{44.61} & \textbf{14.38} &  & 36.53 & \textbf{9.229} \\
% w/o $D(G(z_c, T_c))$ & 41.73 & 11.2 &  & 33.4 & 8.1 \\
% $D(G(z_c, T_c))$ & 43.4 & 10.1 &  & 35.2 & 8.3 \\\bottomrule
% \end{tabular}
% \caption{Ablation Study of Adversarial training to Zero-Shot Learning with respect to Top 1 Accuracy (\%).}
% \label{tb:ablation study_top_1}
% \end{table}  


% \begin{table}[h]
% 	\centering 
% 	\scalebox{0.82}
% 	{
% 		\begin{tabular}{l|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}}
% 			\Xhline{4\arrayrulewidth}
% 			 &\multicolumn{3}{c|}{CUB}  &\multicolumn{3}{c}{NAB} \\\hline
% 			&&&&&&\\[-0.8em]
% 			methods &25\%  &50\%  &100\%   &25\%  &50\%  &100\%\\ 
% 			\Xhline{4\arrayrulewidth}
% 			&&&&&&\\[-0.8em]
% 			ESZSL \cite{romera2015embarrassingly} 	&   27.9   &27.3       &22.7 &28.9&27.8&20.85\\
% 			ZSLNS \cite{Qiao2016}	&  29.2    &29.5      &23.9&28.78&27.27&22.13\\
% 		    ZSLPP \cite{Elhoseiny_2017_CVPR}	&  42.3    &42.0       &36.3&36.9&35.7&\textbf{31.3}\\
% 			GAZSL \cite{Elhoseiny_2018_CVPR}	&  49.7  &48.3 & 40.3&41.6&37.8&31.0\\
% 			CGAZSL 	&    &  &  & & & \\
% 			\Xhline{4\arrayrulewidth}	
% 		\end{tabular}
% 	}
% 	\caption{Zero-Shot Retrieval using mean Average Precision(mAP) (\%) on CUB and NAB with SCS splitting.
% 	}
% 	\vspace{-3mm}
% 	\label{tb:Retrieval}
% \end{table}





% We also compared our method to the state-of-the art attribute-based ZSL methods on three different data sets (AWA2, aPy and SUn datasets).  The first dataset is Animals With Attributes (AWA2)~\cite{lampert2009} of over 30,000 animal images that match 50 classes in Osherson's classic table that describes how humans associate 85 semantic attributes with animal classes. Second dataset is Objects

 
% ============================================================================================= %


% ---------------------------------------------- CVPR-18 Paper ----------------------------------------------------- %

% \subsection{Experiment Setting}
% \noindent \textbf{Datasets:} We evaluated our method with state-of-the-art
% approaches on two benchmark datasets: \emph{Caltech UCSD Birds-2011} (CUB)~\cite{wah2011caltech} and \emph{North America Birds} (NAB)~\cite{Horn2015}. Both are datasets of birds for fine-grained classification. The CUB dataset contains
% 200 categories of bird species with a total of 11,788
% images, and NAB is a larger dataset of birds with 1011 classes and 48,562 images. Elhoseiny \emph{et al.}~\cite{Elhoseiny_2017_CVPR} extended both datasets by adding the Wikipedia article of each class, and they also reorganized NAB to 404 classes by merging subtle
% division of classes, such as ``American Kestrel
% (Female, immature)" and ``American Kestrel (Adult male)". 
% In ~\cite{Elhoseiny_2017_CVPR}, two different split settings were proposed for both datasets, named \emph{Super-Category-Shared} and \emph{Super-Category-Exclusive} splittings, in term of how close the seen classes are related to the unseen ones. For brevity, we denote them as SCS-split and SCE-split. In the scenario of SCS-split, for each unseen class, there exists one or more seen classes that belong to the same parent category. For instance, both ``Cooper's
% Hawk" in the training set and ``Harris's Hawk" in the testing set are under the parent category ``Hawks". Note that the conventional ZSL setting is SCS-split used in ~\cite{akata2016multi, Qiao2016, romera2015embarrassingly, akata2015evaluation}. On the contrary, in SCS-split, the parent categories of unseen classes are exclusive to those of the seen classes. Intuitively, SCE-split is much harder than SCS-split as the relevance between seen and unseen classes is minimized. We follow both split settings to evaluate the capability of our approach. 


% \noindent \textbf{Textual Representation:}
% We use the raw Wikipedia articles collected by~\cite{Elhoseiny_2017_CVPR} for both benchmark datasets.
% Text articles are first tokenized into
% words, the stop words are removed, and porter stemmor~\cite{Porter} is applied to reduce inflected words to their word stem.  Then, Term
% Frequency-Inverse Document Frequency(TF-IDF) feature
% vector~\cite{salton1988term} is extracted. The dimensionalities of TF-IDF features for CUB and
% NAB are 7551 and 13217.

% \noindent \textbf{Visual Features:}
% We extract the visual features from the activations of the part-based FC layer of VPDE-net. All input images are resized to $224 \times 224$ and fed into the VPDE-net. There are seven semantic parts in CUB dataset: ``head", ``back", ``belly", ``breast", ``leg", ``wing", ``tail". NAB dataset contains the same semantic parts except for ``leg". For each part, a 512-dimensional feature vector is extracted. Concatenating those part-based features in order, we obtain the visual representation of the image. The dimensionalities of visual features for CUB and NAB are 3583 and 3072 respectively. 

% The implementation details of our model and the parameter settings can be found in the supplementary material. 

% \subsection{Zero-Shot Recognition}
% \noindent \textbf{Competing Methods:}
% The performance of our method is compared to seven state-of-the-art algorithms: ZSLPP~\cite{Elhoseiny_2017_CVPR}, MCZSL~\cite{akata2016multi}, ZSLNS~\cite{Qiao2016}, ESZSL~\cite{romera2015embarrassingly}, SJE~\cite{akata2015evaluation}, WAC~\cite{elhoseiny2013write}, SynC~\cite{changpinyo2016synthesized}.
% The source code of ZSLPP, ESZSL, and ZSLNS are available online,
% and we get the code of WAC~\cite{elhoseiny2013write} from its author. For MCZSL and SJE, since their source codes are not available,
% we directly copy the highest scores for non-attribute settings
% reported in~\cite{akata2016multi, akata2015evaluation}.


% We conduct the experiments on both SCS and SCE splits on two benchmark datasets to show the performance of our approach.   Note that some of the compared methods are attribute-based methods but applicable in our setting by replacing the attribute vectors with textual features.  Among these methods MCZSL and ZSLPP leverage the semantic parts of birds for visual representations of images. MCZSL directly uses part annotations as strong supervision to extract CNN representation of each semantic part in the test phase. Unlike MCZSL, our approach and ZSLPP are merely based on the detected semantic parts during both training and testing. The performance of the final zero-shot classification is expected to degrade due to less accurate detection of semantic parts compared to manual annotation in MCZSL. Table~\ref{tb:cub2011} shows the performance comparisons on CUB and NAB datasets. Generally, our method consistently outperforms the state-of-the-art methods. On the conventional split setting (SCS), our approach outperforms the runner-up (ZSLPP) by a considerable gap: $6.5\%$ and $5.3\%$ on CUB dataset and NAB dataset, respectively. Note that ZSL on SCE-split remains rather challenging. The fact that there is less relevant information between the training and testing set makes it hard to transfer knowledge from seen classes to unseen classes. Although our method just improves the performance by less than 1\%, we will show the great improvement on the general merit of ZSL in Sec~\ref{sec:gzsl}  

% \setlength{\tabcolsep}{3pt}
% \begin{table}[h]
% 	%\begin{center}
% 	%\vspace{-4mm}
% 	\centering 
% 	\scalebox{0.8}
% 	{
% 		\begin{tabular}{l| K{1.2cm}| K{1.2cm} | K{1.2cm}| K{1.2cm}}
% 			\Xhline{4\arrayrulewidth}
% 			  &\multicolumn{2}{c|}{CUB}  &\multicolumn{2}{c}{NAB}  \\ 
% 			\hline
% 			methods &SCS &SCE   &SCS  &SCE  \\ 
% 	\Xhline{4\arrayrulewidth}
% 			&&&&\\[-0.8em]
% 			MCZSL \cite{akata2016multi}   	&  34.7 & --  &--&--\\
% 			WAC-Linear \cite{elhoseiny2013write}  	&  27.0  &   5.0 &--&--\\	%\hline
% 			WAC-Kernel \cite{elhoseiny2016write}    	&  33.5    & 7.7 & 11.4 &6.0\\	%\hline
% 			ESZSL \cite{romera2015embarrassingly}     	&  28.5   &7.4 &24.3&6.3\\	%\hline
% 			SJE \cite{akata2015evaluation}  & 29.9 & --&--&--\\
% 			ZSLNS \cite{Qiao2016}  	&  29.1   &7.3 &24.5&6.8\\	%\hline
% 			SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 &18.4&3.8\\
% 			SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 &  5.9 &--&--\\
% 			ZSLPP \cite{Elhoseiny_2017_CVPR}    	&  37.2  &9.7 &30.3&8.1\\
% 			GAZSL   	&  \textbf{43.7}  &\textbf{10.3} &\textbf{35.6}&\textbf{8.6}\\
% 			\Xhline{4\arrayrulewidth}
			
% 		\end{tabular}
% 	}
% 	\vspace{1mm}
% 	\caption{
% 		{ Top-1 accuracy (\%) on \textbf{CUB} and \textbf{NAB} datasets with two split settings.}} 
% 	\vspace{-7.5mm}
% 	\label{tb:cub2011}
% \end{table}


% \subsubsection{Ablation Study}
% We now do the ablation study of the effect of the visual pivot regularization(VP) and the GAN. We trained two variants of our model by only keeping the VP or GAN, denoted as VP-only and GAN-only, respectively. Specifically, in the case of only using VP, our model discards the discriminator and thus is reduced to a visual semantic embedding method with VP loss. The generator essentially becomes a mapping function that projects the semantic feature of classes to the visual feature space. It is worth mentioning that compared to previous linear embedding methods~\cite{elhoseiny2013write, romera2015embarrassingly,Qiao2016,Elhoseiny_2017_CVPR} that usually have one or two projection matrices, our generator has a deeper architecture with three projection matrices if we can roughly treat FC layers as project matrices. Additionally, our generator also differs in adding nonlinearity by using Leaky-ReLU and Tanh as the activation function as shown in Fig.~\ref{fig:framework}. 


% Table~\ref{tb:ablation} shows the performance of each setting. Without the visual pivot regularization, the performance drops drastically by 20.91\% (22.83\%vs.43.74\%) on CUB and 11.36\%     
% (24.22\%vs.35.58\%) on NAB, highlighting the importance of the designed VP regularizer to provide a proper explicit supervision to GAN. 
% Interestingly, we observe that only using VP regularizer as the objective of the generator achieves the accuracy of 28.52\% on CUB and 25.75\% on NAB, which are even higher than that of GAN-only model. This observation naturally introduces another perspective of our approach. We can regard our approach as a visual semantic embedding one with the GAN as a constraint. We argue that generative adversarial model and the visual pivot regularization are critically complementary to each other. GAN makes it possible to get rid of the one-to-one mapping existing in previous embedding methods by generating diverse embeddings on descriptions.
% On the other hand, VP regularization attempts to restrict such imaginary samples of the generator within the proper range, thus keeping the discrimination of generated features across the classes. The importance of both components is verified by the superior performance of our complete approach compared to two variants. 
% \begin{table}[h]
	
% 	\centering 
% 	\scalebox{0.8}
% 	{
% 		\begin{tabular}{l|K{1.3cm}|K{1.3cm}|K{1.3cm}|K{1.3cm}}
					
% 			\Xhline{4\arrayrulewidth}
% 			&\multicolumn{2}{c|}{CUB}  &\multicolumn{2}{c}{NAB} \\\hline
% 			&&&&\\[-0.8em]
% 			methods & w/ FC  &w/o FC & w/ FC  &w/o FC\\ 
% 			\Xhline{4\arrayrulewidth}
% 			&&&&\\[-0.8em]
			
% 			GAN-only &  22.83   &21.83 &24.22& 24.80\\
% 			VP-only  &28.52 &26.76 &25.75&23.42\\
% 			GAZSL	&  \textbf{43.74}   &40.85 &\textbf{35.58}&32.94\\
% 			\Xhline{4\arrayrulewidth}	
% 		\end{tabular}
% 	}
% 	%	\vspace{1mm}
% 	\caption{
% 		Effects of different components on zero-shot classification accuracy (\%) on CUB and NAB datasets with SCS split setting.
% 	}
% 	\vspace{-3mm}
% 	\label{tb:ablation}
% \end{table}


% We also analyzed the effectiveness of our additional FC layer on textual features for noise suppression. As shown in Table~\ref{tb:ablation}, in general, our method with FC layer outperforms one without FC layer by $2\%$ to $3\%$ in most cases. The superiority can also be observed in two variants. In practice, the high dimensional TF-IDF feature is compacted to a $1000D$ feature vector. Unlike the traditional dimensionality  reduction technique (e.g., PCA), FC layer contains trainable weights and is optimized in an end-to-end fashion. 



% \begin{figure}
% 	\centering
% 	\subfloat[CUB with SCS splitting]{\includegraphics[width= 1.6in]{figures/GZSL1-crop.pdf}} 
% 	\subfloat[CUB with SCE splitting]{\includegraphics[width= 1.6in]{figures/GZSL2-crop.pdf}}\\
%     \vspace{-2mm}
% 	\subfloat[NAB with SCS splitting]{\includegraphics[width= 1.6in]{figures/GZSL3-crop.pdf}} 
% 	\subfloat[NAB with SCE splitting]{\includegraphics[width= 1.6in]{figures/GZSL4-crop.pdf}}\\
% 	%\subfloat[]{\includegraphics[width= 1.2in]{motion2-crop.pdf}} \quad
% 	%\subfloat[]{\includegraphics[width= 1.2in]{motion3-crop.pdf}}
% 	\setlength\belowcaptionskip{-2.5ex}
% 	\caption{ Seen-Unseen accuracy
% 		Curve on two benchmarks datasets with two split settings}
% 	\label{fig:GZSL_Curve}
%     \vspace{-4mm}
% \end{figure}

% \subsection{Generalized Zero-Shot Learning}
% \label{sec:gzsl}
% The conventional zero-shot recognition considers that queries come from only unseen classes. However, as the seen classes are often the most common objects, it is unrealistic to assume that we will never encounter them during the test phase~\cite{chao2016empirical}
% . Chao \emph{et al.}~\cite{chao2016empirical} presented a more general metric for ZSL that involves classifying images of both seen classes $\mathcal{S}$ and unseen classes $\mathcal{U}$ into $\mathcal{T} = \mathcal{S}\cup\mathcal{U}$. The accuracies are denoted as $A_{\mathcal{S}\to\mathcal{T}}$ and $A_{\mathcal{U}\to\mathcal{T}}$ respectively. They introduced a balancing parameter $\lambda$ to draw Seen-Unseen accuracy Curve(SUC) and use Area Under SUC  to measure the general capability of methods for ZSL. In our case, we use the trained GAN to synthesize the visual features of both training classes and testing classes. The visual features of each class are averaged to obtain the visual pivots. 
% The nearest neighbor strategy to visual pivots is adopted to predict the class label of images. 

% In Fig.~\ref{fig:GZSL_Curve}, we plot SUC and report the AUSUC scores of our method and the competitors. Our method compares favorably to competitors in all cases except on NAB with SCS-split, where very high $A_{\mathcal{S}\to\mathcal{T}}$ and low $A_{\mathcal{U}\to\mathcal{T}}$ indicate that $WAC_{linear}$ is overfitting the dataset. It's worth noting that although our method only slightly outperforms competitors in the zero-shot recognition task with SCE splitting, the AUSUC scores of our method are $42.6\%$ and $56.7\%$ higher than those of the runner-up on CUB and NAB respectively, indicating a superior and balanced performance on $A_{\mathcal{S}\to\mathcal{T}}$ and $A_{\mathcal{U}\to\mathcal{T}}$.



% \subsection{Zero-Shot Retrieval}
% Zero-shot image retrieval is defined as retrieving images giving the semantic representation of an unseen class as the query. We use mean average precision (mAP) to evaluate the performance. In Table~\ref{tb:Retrieval}, we report the performance of different settings: retrieving 25\%, 50\%, 100\% of the number of images for each class from the whole dataset. The precision is defined as the ratio of the number of correct retrieved images to that of all retrieved images.  We adopt the same strategy as in GZSL to obtain the visual pivots of unseen classes. Given the visual pivot, we retrieve images based on the nearest neighbor strategy in $\mathcal{X}$ space.

% \begin{table}[h]
% 	\centering 
% 	\scalebox{0.82}
% 	{
% 		% 		\begin{tabular}{l|c | c | c | c }
% 		\begin{tabular}{l|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}|K{0.9cm}}
% 			% \begin{tabular*}{0.9\linewidth}{@{\extracolsep{\fill}}l|c|c|c|c}
% 			\Xhline{4\arrayrulewidth}
% 			 &\multicolumn{3}{c|}{CUB}  &\multicolumn{3}{c}{NAB} \\\hline
% 			&&&&&&\\[-0.8em]
% 			methods &25\%  &50\%  &100\%   &25\%  &50\%  &100\%\\ 
% 			\Xhline{4\arrayrulewidth}
% 			&&&&&&\\[-0.8em]
% 			ESZSL \cite{romera2015embarrassingly} 	&   27.9   &27.3       &22.7 &28.9&27.8&20.85\\
			
% 			ZSLNS \cite{Qiao2016}	&  29.2    &29.5      &23.9&28.78&27.27&22.13\\
			
% 		ZSLPP \cite{Elhoseiny_2017_CVPR}	&  42.3    &42.0       &36.3&36.9&35.7&\textbf{31.3}\\
			
% 			VP-only&  17.8   &16.4  & 13.9&15.1&13.1&11.5\\
% 			GAN-only	&  18.0   &17.5  & 15.2&21.7&20.3&16.6\\
% 			GAZSL	&  \textbf{49.7 }  &\textbf{48.3} & \textbf{40.3}&\textbf{41.6}&\textbf{37.8}&31.0\\
% 			\Xhline{4\arrayrulewidth}	
% 		\end{tabular}
% 	}
% 	%	\vspace{1mm}
% 	\caption{Zero-Shot Retrieval using mean Average Precision
% (mAP) (\%) on CUB and NAB with SCS splitting.
% 	}
% 	\vspace{-3mm}
% 	\label{tb:Retrieval}
% \end{table}
% Our method outperforms competitors by $4\% \sim 7\%$. 
% We discover that although VP-only performs better than GAN-only on the recognition task, its performance is inferior to GAN-only on retrieval tasks. Without the  constraints of WGAN, VP-only suffers from heavy mode collapse, and synthetic features easily collapse into the visual pivot of each class with less diversity.   

% We also provide qualitative results of our method as shown in Fig.~\ref{fig:retivial}. Each row is one class, and the class name and the precision are shown on the left. The first column is Top-1 within-class nearest neighbor. The following five columns are Top-5 overall nearest neighbors without considering the instances in the first column. 


% \begin{figure}
% \centering
% 	\includegraphics[width=7.8cm,height=6.5cm]{figures/retrivialexample_low.pdf}
% 	\caption{Qualitative results of zero-shot retrieval. The first three rows are classes from CUB and the rest from NAB. Correct and incorrect retrieved instances are shown in green and red respectively.}
% 	\label{fig:retivial}
% 	\vspace{-5mm}
% \end{figure}
% \subsection{t-SNE Demonstration}
% Fig.~\ref{fig:tSNE} demonstrates the t-SNE~\cite{maaten2008visualizing} visualization of the real features, the synthesized features for unseen classes under different settings. Despite some overlaps, the real features roughly distribute in separate clusters w.r.t class labels. The features generated by our method keep the same structure. Ideally, we expect the distribution of generated features matches that of the real ones in $\mathcal{X}$ space.  Empirically, despite that some deviating clusters of synthesized features  due to the bias between testing and training data, many clusters are well aligned to the real ones. Without the VP regularizer, GAN encourages the high diversity of features with no constraints. The features disperse greatly and lack the discrimination across classes.
 
 
 
 
 % ---------------------------------------------- Old Comments ----------------------------------------------------- %
 %We follow the partitioning strategy of~\cite{akata2016label} to split CUBird dataset to \emph{100/50/50} classes for \emph{training/validation/testing} data. For NABird, we use the \emph{242/81/81 Super-Category-Shared} splitting as described in~\cite{Elhoseiny_2017_CVPR}.


%For the sake of fair comparisons, we first compare the performance in the scenario of using ground-truth annotations .
%In all the following experiments, we only used our approach with the detected parts for fair comparisons. 


%SO who is the actual regularization, VP regularization or GAN? Our answer is: BOTH.  
%serves to preserve the diversity of synthesized features inside each class, which gets rid of one-to-one mapping existing in embedding methods.



%The essential idea is to introduce a balance parameter $\lambda$. With the  extremely small initial setting of $\lambda$, data are encouraged to classified to unseen classes. As $\lambda$ increases, data are gradually encouraged to be classified into seen classes. 


%By comparing to two variants, it clearly demonstrate the criticality of the combination of these two mutually complementary components. 
%Some instances are hard to distinguish even for humans. 

==> experiments.tex <==
\section{Experiments and Discussions}
Overall, we investigate the performance of our method on two class-level semantic settings: textual and attribute descriptions. We use several datasets with different scale to verify the reliability of our model. Since the textual based ZSL is a harder problem, we used it to run an ablation study for zero-shot retrieval and generalized ZSL. Then, we conducted experiments for bothe settings to validate the generality of our work (Modify).

\subsection{Network Design with Simplest Settings}
In order to test the performance of our creativity inspired network, we create the simplest setting first. The encoded text $t_k$ is fed to a fully connected layer first to reduce the dimensionality and to suppress the noise before concatenation with $z$. Then we use two fully connected layers for generator and two other connected layers for discriminator. 

\textbf{Cross-Validation} The creativity weight $\lambda$ of our loss is a hyperparameter that we found easy to tune on all of our experiments. We start by split with nearly 80\%-20\% ratio for all settings. Training and validation classes are selected randomly prior to the training. Then, we compute validation performance when training the model on the 80\% split every 100 iterations out of 3000 iterations. We inverstigate a wide range of value for $\lambda$, and the value that scores highest validation performance is selected to be used at the inference time. Finally, we combine training and validation data and evaluate the performance on testing data. (Modify). 

\subsubsection{Wikipedia based ZSL Results (6 or more benchmarks)}
\textbf{Text Representation} Textual features for each class are extracted from corresponding raw Wikipedia articles collected by \cite{elhoseiny2013write}, \cite{elhoseiny2017link}. We used Term Frequency-Inverse Document Frequency (TF-IDF)\cite{salton1988term} feature vector of dimensionality 7551 for CUB and 13217 for NAB. (Talk more about the results of ImageNet)

\begin{table}[!htbp]
% \parbox{.57\linewidth}{
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
WAC-Linear \cite{elhoseiny2013write} & 27.0 & 5.0 & -- & -- &  & 23.9 & 4.9 & 23.5 & -- \\
WAC-Kernel \cite{elhoseiny2016write} & 33.5 & 7.7 & 11.4 & 6.0 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
ESZSL \cite{romera2015embarrassingly} & 28.5 & 7.4 & 24.3 & 6.3 &  & 18.5 & 4.5 & 9.2 & 2.9 \\
ZSLNS \cite{Qiao2016} & 29.1 & 7.3 & 24.5 & 6.8 &  & 14.7 & 4.4 & 9.3 & 2.3 \\
SynC$_{fast}$ \cite{changpinyo2016synthesized} & 28.0 & 8.6 & 18.4 & 3.8 &  & 13.1 & 4.0 & 2.7 & 3.5 \\
% SynC$_{OVO}$ \cite{changpinyo2016synthesized} & 12.5 & 5.9 & -- & -- &  & 1.7 & 1.0 & 0.1 & --\\
ZSLPP \cite{Elhoseiny_2017_CVPR} &  37.2 & 9.7 &30.3 & 8.1 &  & 30.4 & 6.1 & 12.6 & 3.5 \\ \hline
FeatGen~\cite{xian2018feature} &  43.9 & 9.8 &36.2 & 8.7 &  & 34.1 & 7.4 & 21.3 & 5.6 \\
FeatGen\cite{xian2018feature}+ \textbf{CIZSL} &  44.2 $\mathcolor{blue}{\mathbf{ ^{ +0.3}}}$  & 12.1 $\mathcolor{blue}{\mathbf{ ^{+2.3}}}$  & 36.3 $ \mathcolor{blue}{\mathbf{ ^{+0.1}}}$ & \textbf{9.8} $\mathcolor{blue}{\mathbf{ ^{+1.1}}}$ &  & 37.4 $\mathcolor{blue}{\mathbf{ ^{+2.7}}}$ & 9.8$\mathcolor{blue}{\mathbf{ ^{+2.4}}}$ & 24.7$\mathcolor{blue}{\mathbf{ ^{+3.4}}}$ & 6.2 $\mathcolor{blue}{\mathbf{ ^{+0.6}}}$ \\  \hline
GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\ 
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL} & 41.9 $\mathcolor{red}{\mathbf{ ^{-1.8}}}$ & 15.5 $\mathcolor{blue}{\mathbf{ ^{+ 5.2}}}$ & $35.0 \mathcolor{red}{\mathbf{ ^{-0.6}}}$ & 9.6 $\mathcolor{blue}{\mathbf{ ^{+1.0}}}$ & & 39.2 $\mathcolor{blue}{\mathbf{ ^{+3.8}}}$ & 12.6 $\mathcolor{blue}{\mathbf{^{+3.9}}}$ & 22.6 $\mathcolor{blue}{^{\mathbf{ + 2.2}}}$ & 6.9 $\mathcolor{blue}{^{\mathbf{ + 1.1}}}$\\
\bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level textual description from \textbf{CUB} and \textbf{NAB} datasets with two-split setting.}
\label{tb:nab_cub}
% \vspace{-1.67ex}
% }
\end{table}  
% \subsection{Updated Networks with More Complicated Settings}
% \subsubsection{Deeper Connected Networks}
% \subsubsection{Fully Convolutional Networks}
% Think about whether illustrating following the network design sequence or dataset with different scales ?

\section{Journal Extensions}
\subsection{Reproduces and Hyperparameters Selection}
\subsection{Better Network Architectures}
\subsection{Interpolation and Extrapolation of Hallucinated Text of Unseen Classes}
\begin{table}[!htbp]
% \parbox{.57\linewidth}{
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}cccccccccc@{}}
\toprule
Metric & \multicolumn{4}{c}{Top-1 Accuracy (\%)} &  & \multicolumn{4}{c}{Seen-Unseen AUC (\%)} \\ \cmidrule(lr){2-5} \cmidrule(l){7-10} 
Dataset & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} &  & \multicolumn{2}{c}{CUB} & \multicolumn{2}{c}{NAB} \\
Split-Mode & Easy & Hard & Easy & Hard &  & Easy & Hard & Easy & Hard \\ \midrule
GAZSL~\cite{Elhoseiny_2018_CVPR}& 43.7 & 10.3 & 35.6 & 8.6 &  & 35.4 & 8.7 & 20.4 & 5.8 \\    \midrule
GAZSL~\cite{Elhoseiny_2018_CVPR} + \textbf{CIZSL}\\ \cmidrule{1-1}
Interpolate & 41.87 & \textbf{15.48} & 35.01 & \textbf{9.61} & & 39.19 & 12.58 & \textbf{23.59} & \textbf{6.92}\\ \hline
Negative Extrapolate & 43.37 & 14.93 & \textbf{35.32} & 9.28 & & 38.88 & 12.74 & 23.22 & 6.73\\ \hline
Positive Extrapolate & 43.50 & 14.84 & 35.08 & 9.49 & & 39.22 & 12.73 & 23.44& 6.70\\ \hline
Neg\&Pos Extrapolate & \textbf{43.85} & 15.35 & 35.30 & 9.47 & & 39.04 & \textbf{12.95} & 23.44 & 6.81\\ \hline
Interpolate \& Extrapolate & 42.89 & 14.97 & \textbf{35.36} & 9.51 & & \textbf{39.42} & 12.38 & 23.44 & 6.77\\

\bottomrule
\end{tabular}%
}
\caption{Interpolate and extrapolate of hallucinated text. }
\label{tb:extrapolate-fusion-all}
% \vspace{-1.67ex}
% }
\end{table}  


\subsection{Discriminative Loss Between Visual Generations of Hallucinated Text of Unseen Classes}
Here goes the loss design.

\subsection{Generative Loss for Hallucinated Text to The Generator}

\subsection{Semantic-Guided Categorizer}

\subsection{Evaluation on Large Scale ImageNet Dataset}. 


